Multimodal Web Navigation with Instruction-Finetuned Foundation Models

The progress of autonomous web navigation has been hindered by the dependence on billions of exploratory interactions via online reinforcement learning, and domain-specific model designs that make it difficult to leverage generalization from rich out-of-domain data. In this work, we study data-driven offline training for web agents with vision-language foundation models. We propose an instruction-following multimodal agent, WebGUM, that observes both webpage screenshots and HTML pages and outputs web navigation actions, such as click and type. WebGUM is trained by jointly finetuning an instruction-finetuned language model and a vision encoder with temporal and local perception on a large corpus of demonstrations. We empirically demonstrate this recipe improves the agent's ability of grounded multimodal perception, HTML comprehension, and multi-step reasoning, outperforming prior works by a significant margin. On the MiniWoB, we improve over the previous best offline methods by more than 45.8%, even outperforming online-finetuned SoTA, humans, and GPT-4-based agent. On the WebShop benchmark, our 3-billion-parameter model achieves superior performance to the existing SoTA, PaLM-540B. Furthermore, WebGUM exhibits strong positive transfer to the real-world planning tasks on the Mind2Web. We also collect 347K high-quality demonstrations using our trained models, 38 times larger than prior work, and make them available to promote future research in this direction.

==> figure_table_latex/dataset_details.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{1.0}{
\begin{tabular}{l|rrr}
\toprule
\textbf{Task} & \textbf{\# of episodes} & \textbf{\# of steps} & \textbf{Ratio (episode)} \\
\midrule
book-flight & 9999 & 90177 & 2.88\% \\
choose-date & 383 & 1508 & 0.11\% \\
choose-date-easy & 3353 & 12946 & 0.97\% \\
choose-date-medium & 2222 & 8733 & 0.64\% \\
choose-list & 1861 & 3724 & 0.54\% \\
click-button & 9782 & 9909 & 2.82\% \\
click-button-sequence & 10000 & 20000 & 2.88\% \\
click-checkboxes & 9761 & 28904 & 2.81\% \\
click-checkboxes-large & 1962 & 19072 & 0.57\% \\
click-checkboxes-soft & 9228 & 36384 & 2.66\% \\
click-checkboxes-transfer & 10000 & 59793 & 2.88\% \\
click-collapsible & 5947 & 13077 & 1.71\% \\
click-collapsible-2 & 2199 & 5627 & 0.63\% \\
click-color & 2554 & 2554 & 0.74\% \\
click-dialog & 10000 & 10000 & 2.88\% \\
click-dialog-2 & 3285 & 3285 & 0.95\% \\
click-link & 9961 & 9961 & 2.87\% \\
click-menu & 3238 & 3243 & 0.93\% \\
click-option & 9998 & 20000 & 2.88\% \\
click-pie & 3724 & 8548 & 1.07\% \\
click-scroll-list & 0 & 0 & 0.00\% \\
click-shades & 0 & 0 & 0.00\% \\
click-shape & 6116 & 6117 & 1.76\% \\
click-tab & 9978 & 13177 & 2.88\% \\
click-tab-2 & 1844 & 2109 & 0.53\% \\
click-tab-2-hard & 1574 & 1916 & 0.45\% \\
click-test & 10000 & 10000 & 2.88\% \\
click-test-2 & 10000 & 10000 & 2.88\% \\
click-widget & 9963 & 9963 & 2.87\% \\
count-shape & 5849 & 5893 & 1.69\% \\
email-inbox & 5159 & 14258 & 1.49\% \\
email-inbox-forward-nl & 9995 & 39980 & 2.88\% \\
email-inbox-forward-nl-turk & 4900 & 20165 & 1.41\% \\
email-inbox-nl-turk & 4346 & 11416 & 1.25\% \\
enter-date & 10000 & 20000 & 2.88\% \\
enter-password & 9980 & 29940 & 2.88\% \\
enter-text & 10000 & 20000 & 2.88\% \\
enter-text-dynamic & 9983 & 19966 & 2.88\% \\
enter-time & 0 & 0 & 0.00\% \\
focus-text & 10000 & 10000 & 2.88\% \\
focus-text-2 & 10000 & 10000 & 2.88\% \\
grid-coordinate & 8353 & 8353 & 2.41\% \\
guess-number & 1021 & 2042 & 0.29\% \\
identify-shape & 9007 & 9010 & 2.60\% \\
login-user & 9793 & 29379 & 2.82\% \\
login-user-popup & 9786 & 39170 & 2.82\% \\
multi-layouts & 10000 & 40000 & 2.88\% \\
multi-orderings & 10000 & 40000 & 2.88\% \\
navigate-tree & 9864 & 15140 & 2.84\% \\
search-engine & 8872 & 35095 & 2.56\% \\
social-media & 2631 & 4407 & 0.76\& \\
social-media-all & 95 & 208 & 0.03\% \\
social-media-some & 319 & 893 & 0.09\& \\
tic-tac-toe & 3947 & 13773 & 1.14\% \\
use-autocomplete & 3465 & 6930 & 1.00\% \\
use-spinner & 530 & 532 & 0.15\% \\
\midrule
\textbf{Total} & 346827 & 867277 & 100\% \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Details of our multimodal dataset.
It contains about 347K episodes in total.
}
\label{tab:dataset_details}
\end{table}


==> figure_table_latex/dataset_model_size.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{fig/dataset_model.pdf}
\vskip -0.05in
\caption{
Average success rate of \proposedshort{} with different dataset (left) and model sizes (right).
X-axis is a logarithmic scale.
As for both HTML and multimodal models, we could observe the scaling effect: the larger the dataset and model size are, the higher the success rates are.
Surprisingly, our approach outperforms previous SL state-of-the-art (48.4\% by \citet{gur2022html}) more than 9.9\% even with 2.8K-episode dataset (about 25\% of the previous dataset curated by \citet{liu2018wge}). 
See \autoref{sec:dataset_model_details} for further details.
}
\label{fig:dataset_model_size}
\end{figure}

==> figure_table_latex/flan_t5_miniwob_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{llr}
\toprule
\textbf{Pre-Trained Models} & \textbf{Modality} & \textbf{Success Rate} \\
\midrule
% T5-XL & HTML & 49.8\% \\  % re-training with our dataset
T5-XL~\citep{gur2022html} & HTML & 48.4\% \\
T5-XL, ViT-B16 & HTML+Image & 55.6\% \\
\midrule
Flan-T5-XL & HTML & 61.5\% \\
Flan-T5-XL, ViT-B16 & HTML+Image & 66.1\% \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate with different pre-trained models. We refer \citet{gur2022html} for T5-XL result and other models are trained with our 347K-episode dataset.
In both modalities, instruction-finetuned LLM checkpoints (Flan-T5) outperform unsupervised LLM checkpoints (T5) by a large margin (over 10\%).
}
\label{tab:flan_t5_miniwob_results}
\end{table}


==> figure_table_latex/m_token_miniwob_results.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.95}{
\begin{tabular}{llr}
\toprule
\textbf{Methods} & \textbf{Modality}  & \textbf{Success Rate} \\
\midrule
\proposedshort{} & HTML & 61.5\% \\
\proposedshort{}~(white) & HTML+Image & 61.5\% \\
\proposedshort{}~(random) & HTML+Image & 62.2\% \\
\proposedshort{} & HTML+Image & 66.1\% \\
\midrule
\proposedshort{}~(single, $H=2$) & HTML+Image & 63.6\% \\
\proposedshort{}~(multiple, $H=1$) & HTML+Image & 64.8\% \\
\proposedshort{}~(multiple, $H=2$) & HTML+Image & 66.1\% \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate with white/random image inputs, single/multiple visual tokens, and context length ($H=1,2$). All models are initialized with Flan-T5-XL and ViT-B16, and trained with our 347K-episode dataset. The results imply that
\proposedshort{} successfully leverages semantic and spatial information from image modality, and multiple visual tokens from patches could extract much richer features than a single visual token per image.
}
\label{tab:m_token_miniwob_results}
\end{table}


==> figure_table_latex/main_miniwob_results.tex <==
\begin{table*}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{llllrr}
\toprule
\textbf{Methods} & \textbf{Training} & \textbf{Modality} & \textbf{Pre-trained Models} & \textbf{Dataset} & \textbf{Success Rate} \\
\midrule
CC-Net~\citep{humphreys2022data} & SL & DOM+Image & ResNet & 2.4M & 32.0\% \\
WebN-T5~\citep{gur2022html} & SL & HTML & T5-XL & 12K & 48.4\% \\
WGE~\citep{liu2018wge} & SL+RL & DOM & -- & 12K+ & 64.6\% \\
CC-Net~\citep{humphreys2022data} & SL+RL & DOM+Image & ResNet & 2.4M+ & 96.4\% \\
\midrule
\proposedshort{}~(Ours) & SL & HTML & Flan-T5-XL & 347K & 61.5\% \\
\proposedshort{}~(Ours) & SL & HTML+Image & Flan-T5-XL,ViT-B16 & 347K & 66.1\% \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate on MiniWoB++ among 56 tasks. We recalculate the baseline performances referring \citet{humphreys2022data} and \citet{gur2022html}.
See \autoref{sec:per_task_full} for the detailed scores per task.
\proposedshort{} significantly outperforms previous finetuned-LLM approach~\citep{gur2022html} which is state-of-the-art among methods trained with supervised learning (SL). 
When comparing to existing methods that leverage online reinforcement learning (SL+RL), our proposed \proposedshort{} exceeds the baseline from~\citet{liu2018wge}. Despite the superior performance, our SL model is still behind SL+RL state-of-the-art~\citep{humphreys2022data} due to the data coverage in the training dataset and lack of exploration during RL-finetuning. ``+'' in Dataset column means that the number of episodes, required during RL training steps, is not included because no details were described in their works.
}
\label{tab:main_miniwob_results}
\end{table*}


==> figure_table_latex/miniwob_example_email_inbox_forward_nl.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.95\linewidth]{fig/miniwob_example_email_inbox_forward_nl.pdf}
\vskip -0.05in
\caption{
Example episode on MiniWoB++~\citep{shi2017miniwob,liu2018wge} (\texttt{email-inbox-forward-nl}). The agent clicks the email from the proper sender, and types the correct receiver to forward that email, to satisfy the given instruction (e.g. \textit{Find Gisele's email and forward it to Siana, please}).
\proposedshort{} makes use of both HTML and image screenshot information to adapt a pretrained instruction-finetuned foundation model to solve challenging web-based tasks such as this one.
}
\label{fig:miniwob_example}
\end{figure*}


==> figure_table_latex/mm_t5_architecture.tex <==
\begin{figure*}[ht]
%\begin{figure}[ht]
\centering
% \includegraphics[width=0.9\linewidth]{fig/mm_t5_m_token_architecture_230101.pdf}
\includegraphics[width=0.9\linewidth]{fig/mm_t5_m_token_architecture_230112.pdf}
\vskip -0.05in
\caption{
Overview of \proposedshort{}, our multimodal encoder-decoder transformer model. It takes recent $H$-step screenshots ($H=2$), action history, instruction, and HTML as inputs.
Image observations are embedded to tokens per $16 \times 16$-size patch via pre-trained vision transformer (ViT) \citep{dosovitskiy2020vit}). Multimodal language-image tokens are fed into pre-trained T5 encoder-decoder transformer~\citep{2020t5}, and then predict executable actions in text formats.
}
\label{fig:mm_t5_architecture}
%\end{figure}
\end{figure*}


==> figure_table_latex/per_task_diff_miniwob_top_10.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{fig/per_task_performance_diff_top_10.pdf}
\vskip -0.05in
\caption{
Top-10 performance improvement by adding image modality to HTML on 56 tasks from MiniWoB++. We subtract the success rates to compute absolute improvement: \texttt{(Success Rate of \proposedshort{}(HTML+Image)) - (Success Rate of \proposedshort{}(HTML))}.
Image modality seems to be leveraged for multi-step reasoning tasks with page transitions or tasks that require global contexts (e.g. \texttt{tic-tac-toe} or \texttt{grid-coordinate})
See \autoref{sec:per_task_full} and \ref{sec:example_episodes} for the details.
}
\label{fig:per_task_diff_miniwob_top_10}
\end{figure}


==> figure_table_latex/per_task_miniwob_results.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.9}{
\begin{tabular}{l|rr|rrrr}
\toprule
\textbf{Task} & \textbf{\proposedshort{} (HTML)} & \textbf{\proposedshort{} (HTML+Image)} & \textbf{WebN-T5} & \textbf{WGE} & \textbf{CC-Net (SL)} & \textbf{CC-Net (SL\&RL)} \\
\midrule
book-flight & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.87 \\
choose-date & 0.00 & 0.09 & 0.00 & 0.00 & 0.12 & 0.97 \\
choose-date-easy & 0.08 & 0.64 & 0.03 & -- & 0.42 & 0.99 \\
choose-date-medium & 0.04 & 0.34 & 0.00 & -- & 0.26 & 0.99 \\
choose-list & 0.16 & 0.21 & 0.26 & 0.16 & 0.19 & 0.99 \\
click-button & 0.96 & 1.00 & 1.00 & 1.00 & 0.78 & 1.00 \\
click-button-sequence & 1.00 & 0.99 & 1.00 & 0.99 & 0.47 & 1.00 \\
click-checkboxes & 1.00 & 0.99 & 0.96 & 0.98 & 0.32 & 0.98 \\
click-checkboxes-large & 0.00 & 0.10 & 0.22 & 0.68 & 0.00 & 0.71 \\
click-checkboxes-soft & 1.00 & 0.98 & 0.54 & 0.51 & 0.04 & 0.95 \\
click-checkboxes-transfer & 1.00 & 0.99 & 0.63 & 0.64 & 0.36 & 0.99 \\
click-collapsible & 1.00 & 0.97 & 0.00 & 1.00 & 0.81 & 1.00 \\
click-collapsible-2 & 0.44 & 0.46 & 0.00 & 0.65 & 0.17 & 0.98 \\
click-color & 0.29 & 0.37 & 0.27 & 1.00 & 0.82 & 1.00 \\
click-dialog & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\
click-dialog-2 & 0.32 & 0.33 & 0.24 & 1.00 & 0.88 & 1.00 \\
click-link & 0.98 & 1.00 & 1.00 & 1.00 & 0.59 & 0.99 \\
click-menu & 0.23 & 0.38 & 0.37 & -- & 0.22 & 0.94 \\
click-option & 1.00 & 0.99 & 0.37 & 1.00 & 0.21 & 0.99 \\
click-pie & 0.53 & 0.87 & 0.51 & 0.32 & 0.15 & 0.97 \\
click-scroll-list & 0.00 & 0.00 & 0.00 & -- & 0.01 & 0.60 \\
click-shades & 0.00 & 0.00 & 0.00 & 0.22 & 0.04 & 1.00 \\
click-shape & 0.60 & 0.64 & 0.53 & 0.64 & 0.11 & 0.95 \\
click-tab & 1.00 & 0.93 & 0.74 & 0.55 & 0.95 & 1.00 \\
click-tab-2 & 0.20 & 0.24 & 0.18 & 0.64 & 0.27 & 0.98 \\
click-tab-2-hard & 0.21 & 0.20 & 0.12 & -- & 0.19 & 0.98 \\
click-test & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
click-test-2 & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\
click-widget & 0.99 & 1.00 & 1.00 & 0.93 & 0.56 & 1.00 \\
count-shape & 0.64 & 0.69 & 0.41 & 0.59 & 0.21 & 0.85 \\
email-inbox & 0.63 & 0.57 & 0.38 & 0.43 & 0.09 & 1.00 \\
email-inbox-forward-nl & 1.00 & 1.00 & 0.60 & -- &  0.00 & 1.00 \\
email-inbox-forward-nl-turk & 0.69 & 0.54 & 0.33 & -- & 0.00 & 1.00 \\
email-inbox-nl-turk & 0.46 & 0.54 & 0.23 & 0.77 & 0.05 & 1.00 \\
enter-date & 1.00 & 1.00 & 0.00 & 0.00 & 0.02 & 1.00 \\
enter-password & 1.00 & 0.99 & 0.97 & 0.99 & 0.02 & 1.00 \\
enter-text & 1.00 & 0.99 & 0.89 & 1.00 & 0.35 & 1.00 \\
enter-text-dynamic & 1.00 & 0.99 & 0.98 & 1.00 & 0.39 & 1.00 \\
enter-time & 0.00 & 0.00 & 0.00 & 0.52 & 0.04 & 0.97 \\
focus-text & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 \\
focus-text-2 & 1.00 & 1.00 & 1.00 & 1.00 & 0.96 & 1.00 \\
grid-coordinate & 0.85 & 1.00 & 0.49 & 1.00 & 0.66 & 1.00 \\
guess-number & 0.10 & 0.12 & 0.00 & 0.00 & 0.21 & 1.00 \\
identify-shape & 0.94 & 1.00 & 0.88 & 0.90 & 0.68 & 1.00 \\
login-user & 0.98 & 0.98 & 0.82 & 0.99 & 0.00 & 1.00 \\
login-user-popup & 0.99 & 0.98 & 0.72 & -- & 0.02 & 1.00 \\
multi-layouts & 1.00 & 0.99 & 0.83 & 0.99 & 0.00 & 1.00 \\
multi-orderings & 1.00 & 0.99 & 0.88 & 0.99 & 0.00 & 1.00 \\
navigate-tree & 0.98 & 1.00 & 0.91 & 0.99 & 0.32 & 0.99 \\
search-engine & 0.69 & 0.95 & 0.34 & 0.26 & 0.15 & 1.00 \\
social-media & 0.13 & 0.36 & 0.21 & 0.39 & 0.03 & 0.90 \\
social-media-all & 0.00 & 0.02 & 0.00 & 0.01 & 0.00 & 0.75 \\
social-media-some & 0.00 & 0.09 & 0.02 & 0.01 & 0.01 & 0.85 \\
tic-tac-toe & 0.25 & 0.48 & 0.48 & 0.37 & 0.32 & 0.83 \\
use-autocomplete & 0.99 & 0.96 & 0.22 & 0.78 & 0.07 & 1.00 \\
use-spinner & 0.08 & 0.05 & 0.07 & 0.04 & 0.47 & 1.00 \\
\midrule
\textbf{Ave.} & 0.615 & 0.661 & 0.484 & 0.646 & 0.343 & 0.964 \\
\textbf{\# of Tasks} & 56 & 56 & 56 & 48 & 56 & 56 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Per-task average success rate on 56 tasks from MiniWoB++.
Because we omit some duplicated tasks (e.g. ``-nodelay'' tasks) from 62 tasks adopted in \citet{gur2022html}, we recalculate the baseline performances referring \citet{humphreys2022data} and \citet{gur2022html}.
}
\label{tab:per_task_miniwob_results}
\end{table}


==> figure_table_latex/webshop_episodes.tex <==
\begin{table}[ht]
\begin{center}
\tiny
%\begin{small}
%\begin{sc}
\scalebox{1.0}{
\begin{tabular}{l|l}
\toprule
\textbf{Instruction:} \textcolor{blue}{i am looking for dark denim color ethylene} & \textbf{Instruction:} \textcolor{blue}{i would like a xlarge plus red camellia fleece}  \\
\textcolor{blue}{vinyl ultra train of size 10, 3rd generation for men,} &  \textcolor{blue}{jacket that can be machine washed, and price lower} \\
\textcolor{blue}{and price lower than 160.00 dollars} & \textcolor{blue}{than 130.00 dollars}\\
\midrule
\textbf{Action:} \texttt{search}\big[\textcolor{violet}{dark denim color ethylene vinyl ultra} & \textbf{Action:} \texttt{search}\big[\textcolor{violet}{xlarge plus red camellia fleece jacket that} \\
\textcolor{violet}{train of size 10, 3rd generation for men}\big] & \textcolor{violet}{can be machine washed}\big]\\
\textbf{Observation:} & \textbf{Observation:} \\
\textcolor{red}{\big[back to search\big]} \textcolor{olive}{page 1 (total results: 50)} \textcolor{red}{\big[next\big]} &\textcolor{red}{\big[back to search\big]} \textcolor{olive}{page 1 (total results: 50)} \textcolor{red}{\big[next\big]} \\
 & \\
\textcolor{violet}{\big[b08b1mcfkl\big]} & \textcolor{violet}{\big[b09h2qsj5p\big]} \\
\textcolor{teal}{salewa ultra train 3 - men's} &  \textcolor{teal}{men's thermal underwear pants usb heated warm cotton} \\
\textcolor{teal}{\$104.0 to \$182.99} & \textcolor{teal}{with zone 3 heating long trousers leggings bottoms} \\
\textcolor{violet}{\big[b07j5mc2x1\big]} & \textcolor{teal}{\$56.77} \\
\textcolor{teal}{skechers men's low-top trainers, us men} &  \textcolor{violet}{\big[b09hcddf1x\big]} \\ 
\textcolor{teal}{\$53.39 to \$140.35} & \textcolor{teal}{men's thermal underwear pants usb heated warm cotton} \\
\textcolor{violet}{\big[b07x5hr3tz\big]} & \textcolor{teal}{long trousers leggings bottoms for winter washable baselayer}  \\
\textcolor{teal}{bruno marc men's linen canvas stretch loafer shoes} & \textcolor{teal}{\$56.77 to \$56.99} \\
\textcolor{teal}{\$39.99} & \textcolor{violet}{\big[b09jgmr43j\big]} \\
& \textcolor{teal}{premium soft and smooth faux fur loose plush vest jackets} \\
\textbf{Action:} \texttt{click}\big[\textcolor{violet}{b08b1mcfkl}\big] & \textcolor{teal}{fashion sexy fuzzy sleeveless outwear} \\
\textbf{Observation:} &  \textcolor{teal}{\$9.47 to \$12.47} \\
\textcolor{red}{\big[back to search\big]} \textcolor{red}{\big[prev\big]} &  \\
\textcolor{teal}{size \big[7\big]\big[7.5\big]\big[8\big]\big[8.5\big]\big[9\big]\big[9.5\big]\big[10\big]\big[10.5\big]\big[11\big]\big[11.5\big]} & \textbf{Action:} \texttt{click}\big[\textcolor{red}{next}\big] \\
\textcolor{teal}{\big[12\big]\big[12.5\big]\big[13\big]} &  \textbf{Observation:} \\
\textcolor{teal}{color \big[ombre blue \textbar~ red orange\big]\big[raw green \textbar~ black out\big]} & \textcolor{red}{\big[back to search\big]} \textcolor{olive}{page 2 (total results: 50)} \textcolor{red}{\big[prev\big]} \textcolor{red}{\big[next\big]} \\
\textcolor{teal}{\big[dark denim \textbar~ red orange\big]} &  \\
\textcolor{teal}{salewa ultra train 3 - men's} & \textcolor{violet}{\big[b07cqt8rbl\big]} \\
\textcolor{teal}{price: \$104.0 to \$182.99} & \textcolor{teal}{king and queen write hoodie couple matching sweater} \\
\textcolor{teal}{rating: n.a.} & \textcolor{teal}{pullover hooded sweatshirt jacket} \\
\textcolor{teal}{\big[description\big]} \textcolor{teal}{\big[features\big]} \textcolor{teal}{\big[reviews\big]} \textcolor{red}{\big[buy now\big]} & \textcolor{teal}{\$26.99 to \$29.99}  \\
& \textcolor{violet}{\big[b09jmvfpzg\big]} \\
\textbf{Action:} \texttt{click}\big[\textcolor{teal}{dark denim \textbar~ red orange}\big] & \textcolor{teal}{mens sherpa quilted lined flannel jacket plus size plaid} \\
\textbf{Observation:} you have clicked dark denim \textbar~ red orange. & \textcolor{teal}{button down fleece shirts coats thicken warm} \\
& \textcolor{teal}{cotton outwear} \\
\textbf{Action:} \texttt{click}\big[\textcolor{teal}{10}\big] &  \textcolor{teal}{\$36.79 to \$55.99}  \\
\textbf{Observation:} you have clicked 10. &  \textcolor{violet}{\big[b09kxfgbn2\big]} \\
& \textcolor{teal}{mankalvxy womens jacket cardigan flannel cowl neck} \\
\textbf{Action:} \texttt{click}\big[\textcolor{red}{buy now}\big] &   \textcolor{teal}{asymmetric loose outerwear plus size xs-xxl 0-22}  \\
\textbf{Termination:} Your score (min 0.0, max 1.0): 1.0 & \textcolor{teal}{\$20.3 to \$26.85} \\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{violet}{b07cqt8rbl}\big]\\
& \textbf{Observation:} \\
& \textcolor{red}{\big[back to search\big]} \textcolor{red}{\big[prev\big]} \\
& \textcolor{teal}{size \big[king-small\big]\big[queen-small\big]\big[king-medium\big]} \\
& \textcolor{teal}{\big[queen-medium\big]\big[king-large\big]\big[queen-large\big]\big[king-xxl\big]} \\
& \textcolor{teal}{\big[king-xlarge\big]\big[queen-xlarge\big]\big[queen-xxlarge\big]} \\
& \textcolor{teal}{king and queen write hoodie couple matching sweater}  \\
& \textcolor{teal}{pullover hooded sweatshirt jacket}  \\
& \textcolor{teal}{price: \$26.99 to \$29.99} \\
& \textcolor{teal}{rating: n.a.} \\
& \textcolor{teal}{\big[description\big]} \textcolor{teal}{\big[features\big]} \textcolor{teal}{\big[reviews\big]} \textcolor{red}{\big[buy now\big]} \\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{red}{prev}\big]\\
& \textbf{Observation:} \\
& \textcolor{red}{\big[back to search\big]} \textcolor{olive}{page 2 (total results: 50)} \textcolor{red}{\big[prev\big]} \textcolor{red}{\big[next\big]} \\
& \\
& \textcolor{violet}{\big[b07cqt8rbl\big]} \\
& \textcolor{teal}{king and ...} \\
& \textcolor{violet}{\big[b09jmvfpzg\big]} \\
& \textcolor{teal}{mens sherpa ...} \\
& \textcolor{violet}{\big[b09kxfgbn2\big]} \\
& \textcolor{teal}{mankalvxy womens...} \\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{violet}{b09jmvfpzg}\big]\\
& \textbf{Observation:} \\
& \textcolor{red}{\big[back to search\big]} \textcolor{red}{\big[prev\big]} \\
& \textcolor{teal}{color \big[army green\big]\big[black\big]\big[coffee\big]\big[gray\big]\big[green\big]\big[red\big]} \\
& \textcolor{teal}{\big[a-army green\big]\big[a-red\big]} \\
& \textcolor{teal}{size \big[small\big]\big[medium\big]\big[large\big]\big[x-large\big]\big[xx-large\big]} \\
& \textcolor{teal}{\big[3x-large\big]} \\
& \textcolor{teal}{mens sherpa quilted lined flannel jacket plus size plaid button} \\
& \textcolor{teal}{down fleece shirts coats thicken warm cotton outwear} \\
& \textcolor{teal}{price: \$36.79 to \$55.99} \\
& \textcolor{teal}{rating: n.a.} \\
& \textcolor{teal}{\big[description\big]} \textcolor{teal}{\big[features\big]} \textcolor{teal}{\big[reviews\big]} \textcolor{red}{\big[buy now\big]} \\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{teal}{red}\big]\\
& \textbf{Observation:} you have clicked red.\\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{teal}{x-large}\big]\\
& \textbf{Observation:} you have clicked x-large.\\
& \\
& \textbf{Action:} \texttt{click}\big[\textcolor{red}{buy now}\big] \\
& \textbf{Termination:} Your score (min 0.0, max 1.0): 1.0 \\
\bottomrule
\end{tabular}
}
%\end{sc}
%\end{small}
\end{center}
\vskip -0.1in
\caption{Example of successful episodes demonstrated by \proposedshort{} on WebShop~\citep{yao2022webshop}.
\proposedshort{} could search and
choose the required product and choose proper options (left).
In addition, \proposedshort{} could also compare the products with browsing and backtracking (i.e. clicking ``next'' or ``prev'' buttons) during the episodes (right).
}
\label{tab:webshop_episodes}
\end{table}

==> figure_table_latex/webshop_results.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.9}{
\begin{tabular}{lllrr}
\toprule
\textbf{Methods} & \textbf{Training} & \textbf{Models} & \textbf{Score} & \textbf{Success Rate} \\
\midrule
Rule & -- & -- & 45.6 & 9.6\% \\
IL & SL & BART, BERT & 59.9 & 29.1\% \\
IL+RL & SL+RL & BART, BERT & 62.4 & 28.7\% \\
Act & In-context & PaLM-540B & 62.3 & 30.1\% \\
ReAct & In-context & PaLM-540B & 66.6 & 40.0\% \\
WebN-T5 & SL & T5-XL & 61.0 & 29.8\% \\
\midrule
\proposedshort{} & SL & Flan-T5-XL & \textbf{67.5} & \textbf{45.0\%} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{Average score and success rate on WebShop~\citep{yao2022webshop} with 500 trials.
\proposedshort{} achieves 45.0\% success, outperforming baseline approaches including ReAct, a prompted PaLM-540B.
We refer \citet{yao2022react} for the baselines.
}
\label{tab:webshop_results}
\end{table}

==> figure_table_latex_iclr/main_miniwob_results.tex <==
\begin{table*}[t]
\begin{center}
\begin{small}
\scalebox{0.8}{
%\begin{sc}
\begin{tabular}{lllcrr}
\toprule
\textbf{Methods} & \textbf{Modality} & \textbf{Pre-trained Models} & \textbf{Offline} & \textbf{Dataset} & \textbf{Success Rate} \\
\midrule
CC-Net (SL)~\citep{humphreys2022data} & DOM+Image & ResNet & \textcolor{cb_green}{\CheckmarkBold} & 2.4M & 32.0\% \\
WebN-T5~\citep{gur2022html} & HTML & T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 12K & 48.4\% \\
% WebN-T5 & HTML & T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 347K & 49.8\% \\
MM-WebN-T5 & HTML+Image & T5-XL,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 347K & 55.6\% \\
\midrule
\multirow{3}{*}{\proposedshort{}~(Ours)} & HTML+Image & Flan-T5-Base,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 2.8K & 61.1\% \\
 & HTML & Flan-T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 347K & 75.5\% \\
 & HTML+Image & Flan-T5-XL,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 347K & \textbf{80.3}\% \\
\midrule
\midrule
WGE~\citep{liu2018wge} & DOM & -- & \textcolor{cb_red}{\XSolidBrush} & 12K+ & 64.6\% \\
CC-Net (SL+RL)~\citep{humphreys2022data} & DOM+Image & ResNet & \textcolor{cb_red}{\XSolidBrush} & 2.4M+ & \textbf{96.4}\% \\
\bottomrule
\end{tabular}
%\end{sc}
}
\end{small}
\end{center}
\vskip -0.125in
\caption{
Average success rate on MiniWoB++ among 56 tasks. We recalculate the baseline performances referring prior works~\citep{humphreys2022data,gur2022html}.
See \autoref{sec:per_task_full} for the detailed scores per task.
\proposedshort{} significantly outperforms the previous finetuned-LLM with 3B parameters~\citep{gur2022html}, which is the recent best among offline methods, or its multimodal variant (MM-WebN-T5) even with 2.8K dataset and Base-size model (310M parameters).
Scaling dataset and model size, \proposedshort{} is close to reaching the online RL-finetuned state-of-the-art~\citep{humphreys2022data}, despite fully offline training.
``+'' in Dataset column means extra billions of frames are required during the online RL phase.
}
\vskip -0.3in
\label{tab:main_miniwob_results}
\end{table*}

==> figure_table_latex_neurips/compositional_example_results.tex <==
\begin{figure*}[t]

\begin{minipage}[c]{0.575\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_neurips/compositional_example_click_link_button.pdf}
    % \vskip -0.05in
\end{minipage}
\begin{minipage}[c]{0.4\textwidth}
    \begin{center}
    \begin{small}
    \scalebox{0.85}{
    \begin{tabular}{llr}
    \toprule
    \textbf{Methods} & \textbf{Modality} & \textbf{Success Rate} \\
    \midrule
    WebN-T5~\citep{gur2022html} & HTML & 51.0\% \\
    \midrule
    \proposedshort{} & HTML & 74.2\% \\
    \proposedshort{} & HTML+Image & \textbf{78.5}\% \\
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Left)} Example of compositional evaluation on MiniWoB++. We combine two different tasks (\texttt{click-link} and \texttt{click-button}) into a single-page sequential task (\texttt{click-link\_click-button}) at test time. See \autoref{sec:comp_detail} for the details of combinations.
\textbf{(Right)} Average success rate on 6 compositional MiniWoB tasks. \proposedshort{} generalizes combinational tasks better than \citet{gur2022html}, achieving better success rate by over 27.5\% (HTML+Image) or 23.2\% (HTML).
}
\label{fig:compositional_example_results}
\vskip -0.1in
\end{figure*}


==> figure_table_latex_neurips/compositional_perturbation_example.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.475\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_neurips/compositional_example_click_link_button.pdf}
    % \vskip -0.05in
\end{minipage}
\begin{minipage}[c]{0.475\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_neurips/perturbation_example_click_button.pdf}
    % \vskip -0.05in
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Left)} Example of compositional evaluation on MiniWoB++. We combine two different tasks (\texttt{click-link} and \texttt{click-button}) into a single-page sequential task (\texttt{click-link\_click-button}). See \autoref{sec:comp_detail} for the details of combinations.
\textbf{(Right)} Example of input perturbation for MiniWoB++ evaluation.
We prepare three different types of perturbations at test time: adding extra HTML at the top of the original input HTML (left) or at the bottom of HTML (middle), and adding task-irrelevant attributes such as coordinate information (right).
We randomly sample extra HTML from the human-collected 12K dataset~\citep{liu2018wge}.
This example HTML is taken from \texttt{click-button}.
}
\label{fig:compositional_perturbation_example}
\vskip -0.1in
\end{figure*}


==> figure_table_latex_neurips/dataset_model_size.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig_neurips/dataset_model.pdf}
\vskip -0.05in
\caption{
Average success rate of \proposedshort{} with different dataset (left) and model sizes (right).
X-axis is a logarithmic scale.
As for both HTML and multimodal models, we could observe the scaling effect: the larger the dataset and model size are, the higher the success rates are.
% Surprisingly, our approach outperforms previous SL state-of-the-art (48.4\% by \citet{gur2022html}) more than 7.3\% even with 2.8K-episode dataset (about 25\% of the previous dataset curated by \citet{liu2018wge}) and 7.3\% parameters of \citet{gur2022html}. 
See \autoref{sec:dataset_model_details} for further details.
}
\label{fig:dataset_model_size}
\end{figure}

==> figure_table_latex_neurips/flan_t5_miniwob_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{llr}
\toprule
\textbf{Pre-Trained Models} & \textbf{Modality} & \textbf{Success Rate} \\
\midrule
% T5-XL & HTML & 49.8\% \\  % re-training with our dataset
T5-XL~\citep{gur2022html} & HTML & 48.4\% \\
T5-XL, ViT-B16 & HTML+Image & 55.6\% \\
\midrule
Flan-T5-XL & HTML & 75.5\% \\
Flan-T5-XL, ViT-B16 & HTML+Image & 80.3\% \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Average success rate with different pre-trained models. We refer \citet{gur2022html} for T5-XL result and other models are trained with our 347K-episode dataset.
In both modalities, instruction-finetuned LLM checkpoints (Flan-T5) outperform unsupervised LLM checkpoints (T5) by a large margin (about 25\%).
}
\label{tab:flan_t5_miniwob_results}
\end{table}


==> figure_table_latex_neurips/m_token_miniwob_results.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.95}{
\begin{tabular}{llr}
\toprule
\textbf{Methods} & \textbf{Modality}  & \textbf{Success Rate} \\
\midrule
\proposedshort{} & HTML & 61.5\% \\
\proposedshort{}~(white) & HTML+Image & 61.5\% \\
\proposedshort{}~(random) & HTML+Image & 62.2\% \\
\proposedshort{} & HTML+Image & 66.1\% \\
\midrule
\proposedshort{}~(single, $H=2$) & HTML+Image & 63.6\% \\
\proposedshort{}~(multiple, $H=1$) & HTML+Image & 64.8\% \\
\proposedshort{}~(multiple, $H=2$) & HTML+Image & 66.1\% \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{
Average success rate with white/random image inputs, single/multiple visual tokens, and context length ($H=1,2$). All models are initialized with Flan-T5-XL and ViT-B16, and trained with our 347K-episode dataset. The results imply that
\proposedshort{} successfully leverages semantic and spatial information from image modality, and multiple visual tokens from patches could extract much richer features than a single visual token per image.
}
\label{tab:m_token_miniwob_results}
\end{table}


==> figure_table_latex_neurips/m_token_miniwob_results_per_task_diff_miniwob_top_10.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.55\textwidth}
    \begin{center}
    \begin{small}
    \scalebox{0.85}{
    \begin{tabular}{llr}
    \toprule
    \textbf{Methods} & \textbf{Modality}  & \textbf{Success Rate} \\
    \midrule
    \proposedshort{} & HTML & 75.5\% \\
    \proposedshort{}~(white) & HTML+Image & 76.6\% \\
    \proposedshort{}~(random) & HTML+Image & 78.5\% \\
    \proposedshort{} & HTML+Image & 80.3\% \\
    \midrule
    \proposedshort{}~(single, $H=2$) & HTML+Image & 64.2\% \\
    \proposedshort{}~(multiple, $H=1$) & HTML+Image & 64.0\% \\
    \proposedshort{}~(multiple, $H=2$) & HTML+Image & 66.1\% \\
    \bottomrule
    \end{tabular}
    }
    \end{small}
    \end{center}
    % \vskip -0.05in
\end{minipage}
\begin{minipage}[c]{0.45\textwidth}
    \centering
    \includegraphics[width=0.95\linewidth]{fig_neurips/per_task_performance_diff_top_10.pdf}
    % \vskip -0.05in
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Left)} Average success rate with white/random image inputs, single/multiple visual tokens, and history length ($H=1,2$). 
We use Flan-T5-XL for white/random image ablations, and Flan-T5-Base for visual tokens and history length ablations.
The results imply that
\proposedshort{} successfully leverages spatial and temporal information from image modality, and multiple visual tokens from patches could extract much richer features than a single visual token per image.
\textbf{(Right)} Top-10 performance improvement among MiniWoB++ by adding image modality to HTML. We subtract the success rates to compute absolute improvement: \texttt{(Success Rate of \proposedshort{}(HTML+Image)) - (Success Rate of \proposedshort{}(HTML))}.
Image modality is leveraged for multi-step tasks with dynamic page transitions or tasks that require global perception (e.g. \texttt{book-flight} or \texttt{tic-tac-toe}).
See \autoref{sec:per_task_full} and \ref{sec:example_episodes} for the details.
}
\label{fig:m_token_miniwob_results_per_task_diff_miniwob_top_10}
\vskip -0.1in
\end{figure*}


==> figure_table_latex_neurips/main_miniwob_results.tex <==
\begin{table*}[t]
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{lllcrr}
\toprule
\textbf{Methods} & \textbf{Modality} & \textbf{Pre-trained Models} & \textbf{Offline} & \textbf{Dataset} & \textbf{Success Rate} \\
\midrule
CC-Net (SL)~\citep{humphreys2022data} & DOM+Image & ResNet & \textcolor{cb_green}{\CheckmarkBold} & 2.4M & 32.0\% \\
WebN-T5~\citep{gur2022html} & HTML & T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 12K & 48.4\% \\
% WebN-T5 & HTML & T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 347K & 49.8\% \\
MM-WebN-T5 & HTML+Image & T5-XL,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 347K & 55.6\% \\
\midrule
\multirow{3}{*}{\proposedshort{}~(Ours)} & HTML+Image & Flan-T5-Base,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 2.8K & 61.1\% \\
 & HTML & Flan-T5-XL & \textcolor{cb_green}{\CheckmarkBold} & 347K & 75.5\% \\
 & HTML+Image & Flan-T5-XL,ViT-B16 & \textcolor{cb_green}{\CheckmarkBold} & 347K & \textbf{80.3}\% \\
\midrule
\midrule
WGE~\citep{liu2018wge} & DOM & -- & \textcolor{cb_red}{\XSolidBrush} & 12K+ & 64.6\% \\
CC-Net (SL+RL)~\citep{humphreys2022data} & DOM+Image & ResNet & \textcolor{cb_red}{\XSolidBrush} & 2.4M+ & \textbf{96.4}\% \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\caption{
Average success rate on MiniWoB++ among 56 tasks. We recalculate the baseline performances referring prior works~\citep{humphreys2022data,gur2022html}.
See \autoref{sec:per_task_full} for the detailed scores per task.
\proposedshort{} significantly outperforms the previous finetuned-LLM with 3B parameters~\citep{gur2022html}, which is the recent best among offline methods, or its multimodal variant (MM-WebN-T5) even with 2.8K dataset and Base-size model (310M parameters).
Scaling dataset and model size, \proposedshort{} is close to reaching the online RL-finetuned state-of-the-art~\citep{humphreys2022data}, despite fully offline training.
``+'' in Dataset column means extra billions of frames are required during the online RL phase.
}
\label{tab:main_miniwob_results}
\end{table*}


==> figure_table_latex_neurips/miniwob_example_email_inbox_forward_nl.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig_neurips/miniwob_example_email_inbox_forward_nl.pdf}
\vskip -0.05in
\caption{
Example episode on MiniWoB++~\citep{shi2017miniwob,liu2018wge} (\texttt{email-inbox-forward-nl}). The agent clicks the email from the proper sender, and types the correct receiver to forward that email, to satisfy the given instruction (e.g. \textit{Find Gisele's email and forward it to Siana, please}).
\proposedshort{} makes use of both HTML and image screenshot information to adapt a pre-trained instruction-finetuned foundation model to solve challenging web-based tasks.
}
\label{fig:miniwob_example}
\end{figure*}


==> figure_table_latex_neurips/mm_t5_architecture.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.95\linewidth]{fig_neurips/mm_t5_m_token_architecture_230112.pdf}
\vskip -0.05in
\caption{
Overview of \proposedshort{}, our multimodal encoder-decoder transformer model. It takes recent $H$-step screenshots ($H=2$), action history, instruction, and HTML as inputs.
Image observations are embedded to tokens per $16 \times 16$-size patch via pre-trained vision transformer (ViT) \citep{dosovitskiy2020vit}. Multimodal language-image tokens are fed into pre-trained T5 encoder-decoder transformer~\citep{2020t5}, and then predict executable actions in text formats.
}
\label{fig:mm_t5_architecture}
\end{figure*}


==> figure_table_latex_neurips/per_task_diff_miniwob_top_10.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{fig_neurips/per_task_performance_diff_top_10.pdf}
\vskip -0.05in
\caption{
Top-10 performance improvement by adding image modality to HTML on 56 tasks from MiniWoB++. We subtract the success rates to compute absolute improvement: \texttt{(Success Rate of \proposedshort{}(HTML+Image)) - (Success Rate of \proposedshort{}(HTML))}.
Image modality seems to be leveraged for multi-step reasoning tasks with page transitions or tasks that require global contexts (e.g. \texttt{tic-tac-toe} or \texttt{grid-coordinate})
See \autoref{sec:per_task_full} and \ref{sec:example_episodes} for the details.
}
\label{fig:per_task_diff_miniwob_top_10}
\end{figure}


==> figure_table_latex_neurips/per_task_miniwob_results.tex <==
\begin{table}[ht]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.725}{
\begin{tabular}{l|rr|rrrr}
\toprule
\textbf{Task} & \textbf{\proposedshort{} (HTML)} & \textbf{\proposedshort{} (HTML+Image)} & \textbf{WebN-T5} & \textbf{WGE} & \textbf{CC-Net (SL)} & \textbf{CC-Net (SL\&RL)} \\
\midrule
book-flight & 0.48 & 0.98 & 0.00 & 0.00 & 0.00 & 0.87 \\
choose-date & 0.08 & 0.13 & 0.00 & 0.00 & 0.12 & 0.97 \\
choose-date-easy & 1.00 & 1.00 & 0.03 & -- & 0.42 & 0.99 \\
choose-date-medium & 0.57 & 0.60 & 0.00 & -- & 0.26 & 0.99 \\
choose-list & 0.16 & 0.24 & 0.26 & 0.16 & 0.19 & 0.99 \\
click-button & 0.98 & 1.00 & 1.00 & 1.00 & 0.78 & 1.00 \\
click-button-sequence & 1.00 & 1.00 & 1.00 & 0.99 & 0.47 & 1.00 \\
click-checkboxes & 1.00 & 1.00 & 0.96 & 0.98 & 0.32 & 0.98 \\
click-checkboxes-large & 0.98 & 0.99 & 0.22 & 0.68 & 0.00 & 0.71 \\
click-checkboxes-soft & 1.00 & 0.98 & 0.54 & 0.51 & 0.04 & 0.95 \\
click-checkboxes-transfer & 0.99 & 0.99 & 0.63 & 0.64 & 0.36 & 0.99 \\
click-collapsible & 1.00 & 0.98 & 0.00 & 1.00 & 0.81 & 1.00 \\
click-collapsible-2 & 0.94 & 0.95 & 0.00 & 0.65 & 0.17 & 0.98 \\
click-color & 0.27 & 0.34 & 0.27 & 1.00 & 0.82 & 1.00 \\
click-dialog & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\
click-dialog-2 & 0.34 & 0.43 & 0.24 & 1.00 & 0.88 & 1.00 \\
click-link & 1.00 & 1.00 & 1.00 & 1.00 & 0.59 & 0.99 \\
click-menu & 0.41 & 0.37 & 0.37 & -- & 0.22 & 0.94 \\
click-option & 1.00 & 1.00 & 0.87 & 1.00 & 0.21 & 0.99 \\
click-pie & 0.99 & 0.99 & 0.51 & 0.32 & 0.15 & 0.97 \\
click-scroll-list & 0.00 & 0.00 & 0.00 & -- & 0.01 & 0.60 \\
click-shades & 0.00 & 0.00 & 0.00 & 0.22 & 0.04 & 1.00 \\
click-shape & 0.58 & 0.72 & 0.53 & 0.64 & 0.11 & 0.95 \\
click-tab & 1.00 & 1.00 & 0.74 & 0.55 & 0.95 & 1.00 \\
click-tab-2 & 0.94 & 0.95 & 0.18 & 0.64 & 0.27 & 0.98 \\
click-tab-2-hard & 0.57 & 0.95 & 0.12 & -- & 0.19 & 0.98 \\
click-test & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
click-test-2 & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 & 1.00 \\
click-widget & 1.00 & 1.00 & 1.00 & 0.93 & 0.56 & 1.00 \\
count-shape & 0.64 & 0.68 & 0.41 & 0.59 & 0.21 & 0.85 \\
email-inbox & 0.99 & 0.99 & 0.38 & 0.43 & 0.09 & 1.00 \\
email-inbox-forward-nl & 1.00 & 1.00 & 0.60 & -- &  0.00 & 1.00 \\
email-inbox-forward-nl-turk & 1.00 & 1.00 & 0.33 & -- & 0.00 & 1.00 \\
email-inbox-nl-turk & 0.92 & 0.98 & 0.23 & 0.77 & 0.05 & 1.00 \\
enter-date & 1.00 & 1.00 & 0.00 & 0.00 & 0.02 & 1.00 \\
enter-password & 1.00 & 1.00 & 0.97 & 0.99 & 0.02 & 1.00 \\
enter-text & 1.00 & 1.00 & 0.89 & 1.00 & 0.35 & 1.00 \\
enter-text-dynamic & 1.00 & 1.00 & 0.98 & 1.00 & 0.39 & 1.00 \\
enter-time & 0.00 & 0.00 & 0.00 & 0.52 & 0.04 & 0.97 \\
focus-text & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 1.00 \\
focus-text-2 & 1.00 & 1.00 & 1.00 & 1.00 & 0.96 & 1.00 \\
grid-coordinate & 1.00 & 1.00 & 0.49 & 1.00 & 0.66 & 1.00 \\
guess-number & 0.10 & 0.11 & 0.00 & 0.00 & 0.21 & 1.00 \\
identify-shape & 0.90 & 1.00 & 0.88 & 0.90 & 0.68 & 1.00 \\
login-user & 1.00 & 1.00 & 0.82 & 0.99 & 0.00 & 1.00 \\
login-user-popup & 0.97 & 0.99 & 0.72 & -- & 0.02 & 1.00 \\
multi-layouts & 1.00 & 1.00 & 0.83 & 0.99 & 0.00 & 1.00 \\
multi-orderings & 1.00 & 1.00 & 0.88 & 0.05 & 0.00 & 1.00 \\
navigate-tree & 1.00 & 1.00 & 0.91 & 0.99 & 0.32 & 0.99 \\
search-engine & 0.59 & 0.96 & 0.34 & 0.26 & 0.15 & 1.00 \\
social-media & 0.99 & 1.00 & 0.21 & 0.39 & 0.03 & 0.90 \\
social-media-all & 0.09 & 0.31 & 0.00 & 0.01 & 0.00 & 0.75 \\
social-media-some & 0.39 & 0.68 & 0.02 & 0.01 & 0.01 & 0.85 \\
tic-tac-toe & 0.42 & 0.56 & 0.48 & 0.37 & 0.32 & 0.83 \\
use-autocomplete & 0.98 & 0.98 & 0.22 & 0.78 & 0.07 & 1.00 \\
use-spinner & 0.03 & 0.11 & 0.07 & 0.04 & 0.47 & 1.00 \\
\midrule
\textbf{Ave.} & 0.755 & 0.803 & 0.484 & 0.646 & 0.343 & 0.964 \\
\textbf{\# of Tasks} & 56 & 56 & 56 & 48 & 56 & 56 \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Per-task average success rate on 56 tasks from MiniWoB++.
Because we omit some duplicated tasks (e.g. ``-nodelay'' tasks) from 62 tasks adopted in \citet{gur2022html}, we recalculate the baseline performances referring \citet{humphreys2022data} and \citet{gur2022html}.
}
\label{tab:per_task_miniwob_results}
\end{table}


==> figure_table_latex_neurips/perturbation_example_results.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.575\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig_neurips/perturbation_example_click_button.pdf}
    % \vskip -0.05in
\end{minipage}
\begin{minipage}[c]{0.4\textwidth}
    \begin{center}
    \begin{small}
    %\begin{sc}
    \scalebox{0.7}{
    \begin{tabular}{lllr}
    \toprule
    \textbf{Methods} & \textbf{Modality} & \textbf{Perturbation} & \textbf{Success Rate} \\
    \midrule
    WebN-T5 & HTML & Top & 24.7\% \\
    \citep{gur2022html} & & Bottom & 42.8\% \\
     & & Coordinates & 6.4\% \\
    \midrule
    \proposedshort{} & HTML & Top & 53.6\% \\
     & & Bottom & 48.0\% \\
     & & Coordinates & 39.8\% \\
    \midrule
    \proposedshort{} & HTML+Image & Top & \textbf{71.8}\% \\
     & & Bottom & \textbf{64.7}\% \\
     & & Coordinates & \textbf{62.6}\% \\
    \bottomrule
    \end{tabular}
    }
    %\end{sc}
    \end{small}
    \end{center}
\end{minipage}
\vskip -0.05in
\caption{
\textbf{(Left)} Example of input perturbation for MiniWoB++ evaluation, taken from \texttt{click-button}.
We prepare three different types of perturbations at test time: adding extra HTML at the top of the original input HTML (left) or at the bottom (middle), and adding task-irrelevant attributes in each element (right) such as coordinate information (left, right, top, bottom).
We randomly sample extra HTML from the 12K dataset~\citep{liu2018wge}.
\textbf{(Right)} Average success rate of perturbation evaluation over MiniWoB++ 56 tasks. The results reveal that while all the methods are affected by input corruptions to some extent, \proposedshort{}, especially with multimodality, achieves significantly better performances than previous finetuned-LLM.
}
\label{fig:perturbation_example_results}
\vskip -0.1in
\end{figure*}


==> figure_table_latex_neurips/priorworks.tex <==
\begin{table*}[ht]
\begin{center}
\begin{small}
\scalebox{0.9}{
%\begin{sc}
\begin{tabular}{llcllc}
\toprule
\textbf{Methods} & \textbf{Architecture} & \textbf{Pre-trained} & \textbf{Input} & \textbf{Output} & \textbf{Offline} \\
\midrule
WGE~\citep{liu2018wge} & LSTM, self-attention & \textcolor{cb_red}{\XSolidBrush}$^{~}$ & DOM & Logit of action & \textcolor{cb_red}{\XSolidBrush} \\
CoDE~\citep{gur2018learning,gur2021gminiwob} & Bi-LSTM & \textcolor{cb_red}{\XSolidBrush}$^{~}$ & DOM & Logit of action & \textcolor{cb_red}{\XSolidBrush} \\
DOM-Q-NET\citep{jia2018domqnet} & GNN & \textcolor{cb_red}{\XSolidBrush}$^{~}$ & DOM & Logit of action & \textcolor{cb_red}{\XSolidBrush} \\
CC-Net~\citep{humphreys2022data} & LSTM, Transformer, ResNet & \textcolor{cb_red}{\XSolidBrush}$^{*}$ & DOM, Screenshot & Logit of action & \textcolor{cb_red}{\XSolidBrush} \\
WebShop~\citep{yao2022webshop} & BERT, BART & \textcolor{cb_green}{\CheckmarkBold}$^{~}$ & Text (from HTML) & Logit of action & \textcolor{cb_red}{\XSolidBrush} / \textcolor{cb_green}{\CheckmarkBold} \\
% WebN-T5~\citep{gur2022html} & T5 transformer & \textcolor{cb_green}{\CheckmarkBold}$^{~}$ & HTML & Text & \textcolor{cb_green}{\CheckmarkBold} \\
\midrule
\proposedshort{} (Ours) & T5 Transformer, ViT & \textcolor{cb_green}{\CheckmarkBold}$^{~}$ & HTML, Screenshot & Text & \textcolor{cb_green}{\CheckmarkBold} \\
\bottomrule
\end{tabular}
%\end{sc}
}
\end{small}
\end{center}
\vskip -0.1in
\caption{Prior works have studied web navigation problem as online RL to learn the optimal action distribution with task-specific model architectures from scratch ($^{*}$or partially using pre-trained vision encoder). We omit the web-specialized architecture and input-output space, and convert web navigation into visual question-answering format (text, image $\rightarrow$ text), which allows us to learn the agents offline by leveraging pre-trained foundation models~\citep{2020t5,chung2022flant5,dosovitskiy2020vit} in vision or language domains as strong inductive bias for web environments.
}
\label{tab:priorworks}
\end{table*}


==> figure_table_latex_neurips/webshop_results.tex <==
\begin{table}[t]
\begin{center}
\begin{small}
%\begin{sc}
\scalebox{0.9}{
\begin{tabular}{lllrr}
\toprule
\textbf{Methods} & \textbf{Training} & \textbf{Models} & \textbf{Score} & \textbf{Success Rate} \\
\midrule
Rule & -- & -- & 45.6 & 9.6\% \\
IL & SL & BART, BERT & 59.9 & 29.1\% \\
IL+RL & SL+RL & BART, BERT & 62.4 & 28.7\% \\
Act & In-context & PaLM-540B & 62.3 & 30.1\% \\
ReAct & In-context & PaLM-540B & 66.6 & 40.0\% \\
\midrule
WebN-T5 & SL & T5-XL & 61.0 & 29.8\% \\
\proposedshort{} & SL & Flan-T5-XL & \textbf{67.5} & \textbf{45.0\%} \\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Average score and success rate on WebShop~\citep{yao2022webshop}.
\proposedshort{} achieves 45.0\% success, outperforming baseline approaches including ReAct, a prompted PaLM-540B.
We refer \citet{yao2022react} for the baselines.
}
\label{tab:webshop_results}
\end{table}

